Effective Eigendecomposition based Graph Adaptation for Heterophilic Networks

Graph Neural Networks (GNNs) exhibit excellent performance when graphs have strong homophily property, i.e. connected nodes have the same labels. However, they perform poorly on heterophilic graphs. Several approaches address the issue of heterophily by proposing models that adapt the graph by optimizing task-specific loss function using labelled data. These adaptations are made either via attention or by attenuating or enhancing various low-frequency/high-frequency signals, as needed for the task at hand. More recent approaches adapt the eigenvalues of the graph. One important interpretation of this adaptation is that these models select/weigh the eigenvectors of the graph. Based on this interpretation, we present an eigendecomposition based approach and propose EigenNetwork models that improve the performance of GNNs on heterophilic graphs. Performance improvement is achieved by learning flexible graph adaptation functions that modulate the eigenvalues of the graph. Regularization of these functions via parameter sharing helps to improve the performance even more. Our approach achieves up to 11% improvement in performance over the state-of-the-art methods on heterophilic graphs.

==> sections/behaviour.tex <==
%\section{Behaviour of Heterophilic Graphs - 1 page}
\section{Empirical analysis with motivation for our approach}
%\begin{enumerate}
%    \item Discuss the approach of understanding the behaviour of Heterophilic Graphs
%    \item Task performance plots
%    \item Learnt Weight plots
%    \item Learning desired filter shapes can be difficult with limited labeled data for heterophilic graphs
%\end{enumerate}




\begin{enumerate}
    \item Write down the basic SVD(A) model for exploring and gaining insights into important/relevant eigen vectors.
    \item Give a couple of weight plots - one each from Chameleon and Squirrel dataset. Possibly, connect with observations made in other work. 
    \item Suggest using learned weights as a way to modulate the eigen values. But, not sure whether we can do some simple experiment to validate this idea. 
\end{enumerate}
%The GPR-GNN model performs quite well on homophilic graphs and achieves improved performance on heterophilic graphs.





==> tex/Section4_V1.tex <==
\section{Proposed Approach: Eigen Network Models}
\label{sec:proposedapproach}
In this section, we present an alternate interpretation of the \gprgnn~model and suggest a simple eigendecomposition based graph adaptation approach. We present several model variants each one of them is motivated by considering different aspects of the problem, as we explain below.
\subsection{Eigen Network Model} 
We start by observing closely the GPR component output given by: 
\begin{equation}
    {\mathbf S} = \eigenU h_K(\adjS) \eigenU^T {\mathbf Z}^{(0)}.
\label{eqn:GPRGNN2}    
\end{equation}
Our first observation is that learning filter coefficients is equivalent to learning a \textit{new} graph, ${\tilde \adj(\eigenU, \adjS;\alpha})$ which is dependent on the fixed set of eigenvectors and eigenvalues, but, parameterised using $\alpha$. Therefore, the \gprgnn~model may be interpreted as adapting the original adjacency matrix $\adj$. 
%and is related to several other graph learning methods (e.g., graph attention networks). However, each graph learning method parameterises the graph differently.  

Next, as noted in the previous section, using the structures present in eigendecomposition and polynomial function we can expand (\ref{eqn:GPRGNN2}) by unrolling over eigenvalues and interchanging the summation as; 
\begin{equation}
    {\mathbf S} = \sum_{j=1}^n \eigenUc_j h_K(\adjSv_j;\alpha) \eigenUc^T_j {\mathbf Z}^{(0)}.
\label{eqn:GPRGNN3}    
\end{equation}
Since $h_K(\adjSv_j;\alpha)$ is dependent only on $(\adjSv_j;\alpha)$ our proposal is to replace the polynomial function with any general smooth function, $C(\sigma_i;\alpha)$, which need not be a polynomial and we call $C(\cdot)$ as \textit{graph adaptation} function. We discuss several choices of such functions shortly. The second observation is that (\ref{eqn:GPRGNN2}) is essentially a single layer network. However, the main difficulty arises when the graph parameters are jointly learned with the nonlinear feature transformation and classifier model weights. This is because the embedding computation via (\ref{eqn:GPRGNN2}) involves dense matrix multiplications and are computationally expensive. We can reduce the computational cost in several ways as follows. 
\begin{enumerate}
    \item We use raw input features $\feat$. This helps to pre-compute projected features, $\eigenU^T \feat$. The other possibility is to use pre-trained feature embedding and use $\eigenU^T {\mathbf Z}^{(L)}$. 
    \item It also helps to reduce the dimension of input feature embedding or raw features, Whenever the dimension of raw features or pre-trained embedding is high. We give more details in Section~\ref{sec:EigenEigen}.
    \item Since we are adapting the eigenvalues we may not need a large number of eigenvectors to get good performance.
\end{enumerate}
For ease of discussion, we work with raw features. However, the following approach holds for pre-trained embedding as well. 
Let us rewrite (\ref{eqn:GPRGNN2}) in matrix form as:
\begin{equation}
    {\mathbf S} = \eigenU C(\adjS;\alpha) \eigenU_x
\label{eqn:eigenn}
\end{equation}
where $\eigenU_x = \eigenU^T \feat$. We refer to (\ref{eqn:eigenn}) as \eigennet~as it involves eigenvectors and learnable graph adaptation function that is dependent on eigenvalues. This network forms the basis of our eigendecomposition based modeling approach. 

{\bf Choice of Graph Adaptation Function.} We use graph adaptation function that is a function of eigenvalue and is non-negative. One such function is: $C(\adjSv;\alpha) = \textsc{ReLu}(\alpha_1) \adjSv^{\tilde \alpha_2}$ where $\tilde \alpha_2 = \textsc{ReLu}(\alpha_2)$. A composition of non-negative linear and exponent scaling functions is quite flexible and helps to adapt for graphs having diverse eigenvalue decay rates. Note that we recover original eigenvalues when $\alpha_1 = 1$ and $\alpha_2 = 1$. Another choice is:   $C(\adjSv;\alpha) = \textsc{Sigmoid}(\alpha_1) \adjSv^{\tilde \alpha_2}$. We experimented with both functions and found the former to be better. There may be other choices of graph adaptive functions that perform better. From a practical viewpoint, several functions can be evaluated with the best function selected using traditional hyperparameter optimization strategy.  

{\bf Remarks.} We observe that the learned graph is nothing but $\adj(\alpha) = \eigenU{\mathbf C}(\adjS;\alpha)\eigenU^T$ and is dense with all nodes in the graph are essentially used to learn node embedding. Unlike $\adj^K$, the learned graph can have negative edges and they are optimized using labeled data. This capability to have negative edges enable our \eigennet~model to perform better on heterophily graphs, as we demonstrate in the experimental section. It is worth noting that the necessity of negative edges has been highlighted in~\citet{fagcn} and~\citet{gprgnn} using graph filtering concept. \citet{fagcn} use attention mechanism to learn negative edges. On the other hand, \citet{gprgnn} uses polynomial function with negative weights to obtain negative edges; however, \gprgnn~is constrained to use powers of adjacent matrices with non-negative edges. Furthermore, any graph weighted with negative coefficient ($\alpha_k$) will have all negative edges, and this constraint may limit the capability of \gprgnn. In contrast, our approach to learn negative edges is quite different. It emerges from adapting eigengraphs ($\eigenUc_j\eigenUc_j^T$) starting with good initialization obtained from approximating the graph using eigendecomposition. Our experimental results show that the proposed approach is highly powerful and outperforms both \fagcn~and \gprgnn~on several heterophily datasets.    

\subsection{\label{sec:EigenEigen} Eigen-Eigen Network Model}
It is often useful to reduce dimension of raw features using principal component analysis. Let  ${\mathbf Q} \adjS_x {\mathbf Q}^T$ be the eigendecomposition of $\feat\feat^T$.  
%Let ${\mathbf X} = {\mathbf Q}_x {\mathbf \Sigma}_x {\tilde \mathbf Q}^T_x$ be the singular value decomposition of ${\mathbf X}$. Note that ${\mathbf X}$ is usually any general matrix. 
Using this decomposition, we define parameterised node embedding for $\feat$ as: ${\tilde \feat}(\beta) = {\mathbf Q} {\mathbf C}_x(\adjS_x;\beta)$. Upon substituting node embedding for raw features in the \eigennet~model (\ref{eqn:eigenn}), we get: 
\begin{equation}
    {\mathbf S} = \eigenU {\mathbf C}(\adjS;\alpha) \eigenU_{\tilde x} {\mathbf C_x}(\adjS_x;\beta)
\label{eqn:eigeignn}
\end{equation}
where $\eigenU_{\tilde x} = \eigenU^T {\mathbf Q}$. We refer (\ref{eqn:eigeignn}) as \eigeneigennet~as it involves eigenvectors of both $\adj$ and $\feat$, and, involves learning weights for eigenvectors. Making use of the fact that ${\mathbf C}(\cdot)$ and ${\mathbf C_x}(\cdot)$ are diagonal, we rewrite (\ref{eqn:eigeignn}) as:   
\begin{equation}
    {\mathbf S} = \eigenU {\mathbf F}(\cdot;\alpha,\beta)
\label{eqn:eigeignn2}
\end{equation}
where ${\mathbf F}(\cdot;\alpha,\beta) = {\mathbf U}_{\tilde x} \bigodot {\mathbf c}(\adjS;\alpha) {\mathbf c}^T_x(\adjS_x;\beta)$ and $\bigodot$ denote element-wise product operation. ${\mathbf c}(\cdot)$ and ${\mathbf c}_x(\cdot)$ denote vectors of diagonal entries. Model learning involves learning $({\mathbf W}_c,\alpha, \beta)$ using labeled data by optimizing cross-entropy loss function. In this paper, we are primarily interested in adapting the graph. Therefore, we optimize only $({\mathbf W}_c,\alpha)$ in (\ref{eqn:eigeignn2}), keeping ${\mathbf C}_x$ fixed to eigen values. We leave conducting an experimental study with $\beta$ optimization as a future work. 

\subsection{Eigen-Concat Models} [{\bf To be written}]

Suggest as an alternative to aggregation model with some motivation from (a) \lgcn/\hetegcn~work and (b) how disagreement in $\adj$ and $\feat$~can hurt each other, and say concat model may be beneficial in some situation as disagreements may be easy to resolve in concat model by giving feature importance weight. 

\subsection{Tied-Eigen Model}
\label{sec:tiedeigen}
We propose a regularization for the $\alpha$ variables in the graph adaptation function. Since we are learning from limited labelled data, there is a possibility that we might overfit the training data if we have independent $\alpha$ per eigenvalue. To mitigate this issue, we propose a regularization based on weight tying. Weight tying is essentially assigning the same weight to a group of variables. Weight tying is a popular mechanism of regularization used in CNN~\citep{cnn}, statistical relational learning~\citep{srl}, Markov logic networks~\citep{mln}, probabilistic soft logic~\citep{psl}, language models~\citep{transformer} etc. In Figure~\ref{fig:weightPlots}, we observe that nearby eigenvalues tend to have similar importance. Based on this observation, we divide the sorted set of eigenvalues in fixed-length bins and assign one $\alpha$ variable to each bin. We call this model as \tiedeigen. This allows us to reduce the number of learnable parameters in the model and offer a simple but effective regularization.

\subsection{Model Training and Complexity} Let $p(\cdot;{\mathbf W},\alpha)$ and ${\bf y}$ denote the model predicted probability vector and 1-hot binary representation of true class label. We use the following standard cross-entropy based loss function: 
\begin{equation}
    {\mathcal L}({\mathbf W},\alpha) = -\sum_{i \in {\bf T}} \sum_{j = 1}^m y_{i,j} \log p_{i,j}(\cdot;{\mathbf W},\alpha)
\label{eqn:objfn}
\end{equation}
where ${\bf T}$ and $m$ denote the set of labeled examples and number of classes respectively, and indices $i$ and $j$ index examples and classes respectively. As explained earlier, the model predicted probabilities are computed using \textsc{Softmax} function on classifier model scores, ${\mathbf S} {\mathbf W}_C$. Note that the node embedding matrix (${\mathbf S})$ and its parameterization vary across models, and (\ref{eqn:objfn}) is an instance with parameters indicated for our models. 

Let $J_a$ and $J_x$ denote the number of eigen components used in our model. Assume that the graph adaptive function is parameterized with $J_g$ parameters for each of the $J_x$ component. Then, the number of model parameters needed in the \eigennet~model (\ref{eqn:eigeignn2}) is $J_g J_a + J_x$. As explained earlier, we do not optimize $\beta$ in our graph adaptation experiments. Given ${\mathbf U}_{\tilde x}$, the cost of computing ${\mathbf F}(\cdot)$ in (\ref{eqn:eigeignn2}) is $J_a J_d$. Likewise, given ${\mathbf U}$, the embedding computing cost per node is $J_a J_x$. Since (\ref{eqn:eigeignn2}) requires fresh computation whenever ${\mathbf F}(\cdot)$ is updated, our method is computationally expensive compared to the \gprgnn~method.     

% \begin{enumerate}
    %\item Motivating the approach
    %\item Discuss Concatenation and Aggregation
    %\item Tied Weight Regularization (Prior works in tied weights \url{https://ojs.aaai.org/index.php/AAAI/article/view/11785})
    %\item Various modeling approach:
    %\begin{enumerate}
    %    \item Concat [SVD(NN), NF] + MLP
    %    \item Concat [SVD(NN) NF] + alpha tuning + MLP
    %    \item Concat [SVD(NN) SVD(NF)] + alpha tuning + MLP
    %    \item Concat Simple grouping approach to tying parameters
    %    \item Aggregation [SVD(NN)NF] + MLP
    %    \item Aggregation [SVD(NN)NF] + alpha tuning + MLP
    %    \item Aggregation [SVD(NN)SVD(NF)] + alpha tuning + MLP
    %    \item Aggregation Simple grouping approach to tying parameters
    %\end{enumerate}
    %\item Brief introduction of the section 
    %\item Introduce the modeling approach starting with GPR-GNN model and talk about tuning singular values. Emphasize the single layer network architecture. 
    %\item Explain computational difficulty that arises while using GPR-GNN model - both linear and non-linear features (involving matrix multiplication during training). 
    %\item Motivate use of SVD of X or pre-trained non-linear features and write down our simplified SVD based neighborhood aggregation model involving SVs of both adjacency and feature matrices. 
    %\item Briefly discuss choices of functions used for tuning singular values. 
    %\item Move to Concat model - suggest as an alternative to aggregation model with some motivation from (a) LightGCN/HeteGCN work and (b) how disagreement in A and X can hurt each other, and say concat model may be beneficial in some situation as disagreements may be easy to resolve in concat model by giving feature importance weight. 
    %\item Give a formal defintion of loss function used for training. 
    %\item Briefly talk about model complexity and Computational cost. 
% \end{enumerate}


